Revisiting the Importance of Amplifying Bias for Debiasing

In image classification, "debiasing" aims to train a classifier to be less susceptible to dataset bias, the strong correlation between peripheral attributes of data samples and a target class. For example, even if the frog class in the dataset mainly consists of frog images with a swamp background (i.e., bias-aligned samples), a debiased classifier should be able to correctly classify a frog at a beach (i.e., bias-conflicting samples). Recent debiasing approaches commonly use two components for debiasing, a biased model $f_B$ and a debiased model $f_D$. $f_B$ is trained to focus on bias-aligned samples (i.e., overfitted to the bias) while $f_D$ is mainly trained with bias-conflicting samples by concentrating on samples which $f_B$ fails to learn, leading $f_D$ to be less susceptible to the dataset bias. While the state-of-the-art debiasing techniques have aimed to better train $f_D$, we focus on training $f_B$, an overlooked component until now. Our empirical analysis reveals that removing the bias-conflicting samples from the training set for $f_B$ is important for improving the debiasing performance of $f_D$. This is due to the fact that the bias-conflicting samples work as noisy samples for amplifying the bias for $f_B$ since those samples do not include the bias attribute. To this end, we propose a simple yet effective data sample selection method which removes the bias-conflicting samples to construct a bias-amplified dataset for training $f_B$. Our data sample selection method can be directly applied to existing reweighting-based debiasing approaches, obtaining consistent performance boost and achieving the state-of-the-art performance on both synthetic and real-world datasets.

==> tables/ablation_align_conflict_b_test.tex <==


\begin{table}
\centering
\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{0.3em}
\def\arraystretch{1.2}% 
\begin{tabular}{c | c | c c c c | c c c c}
% \hline\noalign{\smallskip}
\toprule 
\# of bias-aligned     & 100\% & 80\% & 60\% & 40\% & 20\% & 100\% & 100\% & 100\% & 100\% \\
\# of bias-conflicting & 100\% & 20\% & 20\% & 20\% & 20\% & 80\%  & 60\%  & 40\%  & 20\%  \\
\midrule
Colored MNIST          & 58.48\stdv{2.78} & 79.82\stdv{0.65} & 75.75\stdv{5.10} & 73.86\stdv{2.31} & 63.21\stdv{2.86} &  66.47\stdv{2.86} & 73.87\stdv{2.55} & 77.87\stdv{3.30} & 81.58\stdv{0.68} \\
BFFHQ                  & 62.10\stdv{0.79} & 78.52\stdv{1.19} & 75.88\stdv{2.57} & 72.2\stdv{0.88} & 69.12\stdv{1.12} & 69.88\stdv{0.83} &  73.96\stdv{2.44} & 77.6\stdv{1.72} & 79.36\stdv{1.43} \\
Dogs\&Cats          & 53.1\stdv{4.80} & 71.8\stdv{2.04} & 63.86\stdv{4.49} & 60.58\stdv{2.18} & 60.78\stdv{3.53} & 61.18\stdv{3.70} & 71.00\stdv{2.85} & 75.38\stdv{3.27} & 79.22\stdv{2.83} \\
\bottomrule
\end{tabular}}
\caption{Test set accuracy resulting from different number of bias-aligned and bias-conflicting samples in the bias-amplified dataset $\mathcal{D}_A$ for training biased model $f_B$. These results are evaluated on the same bias severity setting (1.0\%).}
\label{tab:ablation_align_conflict_b_test}
\end{table}




==> tables/ablation_align_conflict_prev.tex <==


\begin{table}[t]
\centering
\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{0.3em}
\def\arraystretch{1.2}% 
\begin{tabular}{c | c | c c c c | c c c c}
% \hline\noalign{\smallskip}
\toprule 
\# of B.A.     & 100\% & 80\% & 60\% & 40\% & 20\% & 100\% & 100\% & 100\% & 100\% \\
\# of B.C.     & 100\% & 20\% & 20\% & 20\% & 20\% & 80\%  & 60\%  & 40\%  & 20\%  \\
\midrule
Colored MNIST          & 58.48\stdv{2.78} & \textbf{79.82}\stdv{0.65} & 75.75\stdv{5.10} & 73.86\stdv{2.31} & 63.21\stdv{2.86} &  66.47\stdv{2.86} & 73.87\stdv{2.55} & 77.87\stdv{3.30} & \textbf{81.58}\stdv{0.68} \\
BFFHQ                  & 62.10\stdv{0.79} & \textbf{78.52}\stdv{1.19} & 75.88\stdv{2.57} & 72.2\stdv{0.88} & 69.12\stdv{1.12} & 69.88\stdv{0.83} &  73.96\stdv{2.44} & 77.6\stdv{1.72} & \textbf{79.36}\stdv{1.43} \\
Dogs\&Cats          & 53.1\stdv{4.80} & \textbf{71.8}\stdv{2.04} & 63.86\stdv{4.49} & 60.58\stdv{2.18} & 60.78\stdv{3.53} & 61.18\stdv{3.70} & 71.00\stdv{2.85} & 75.38\stdv{3.27} & \textbf{79.22}\stdv{2.83} \\
\bottomrule
\end{tabular}}
\vspace{0.2cm}
\caption{Test set accuracy of resulting from different number of bias-aligned~(B.A.) and bias-conflicting~(B.C.) samples computed as a ratio in the bias-amplified dataset $\mathcal{D}_A$ for training biased model $f_B$ of LfF. These results are evaluated on the same bias severity setting (1.0\%).}
\vspace{-0.8cm}
\label{tab:ablation_align_conflict}
\end{table}




==> tables/ablation_detecting_performance.tex <==
\begin{table}
\centering
\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{1.0em}
\begin{tabular}{c | c c | c c | c c | c c | c c}
% \hline\noalign{\smallskip}
\toprule 

% Method & $\rho$ & $M$ & Colored MNIST & BFFHQ & Dogs \& Cats & BAR \\
\multicolumn{1}{c|}{\multirow{2}{*}{Method}}
&{\multirow{2}{*}{$\rho$}}
& \multicolumn{1}{c|}{\multirow{2}{*}{$M$}}
& \multicolumn{2}{c}{Colored MNIST}
& \multicolumn{2}{c}{BFFHQ}
& \multicolumn{2}{c}{Dogs \& Cats}
& \multicolumn{2}{c}{BAR}
\\ \cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11} 
% \\ \midrule
% \multicolumn{3}{c}{}
& & & AUROC & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC & AUPRC \\
\midrule
LfF & - & - & 87.26\stdv{8.05} & 22.44\stdv{35.30} & 67.61\stdv{2.42} & \textbf{18.42}\stdv{1.74} & 62.14\stdv{1.81} & 7.22\stdv{2.01} & 48.77\stdv{0.93} & 0.78\stdv{0.00} \\
\midrule
\multirow{3}{*}{BE}
        & 1 & 1 & 89.72\stdv{5.87} & 23.59\stdv{36.90} & 80.01\stdv{4.13} & 4.14\stdv{1.35} & 86.94\stdv{1.93} & 5.32\stdv{0.31} & 68.62\stdv{6.59} & 4.96\stdv{2.55} \\
        & 5 & 5 & 97.45\stdv{2.64} & 26.14\stdv{13.39} & 81.93\stdv{0.26} & 2.88\stdv{0.38} & 82.60\stdv{1.30} & 2.85\stdv{0.19} & \textbf{78.80}\stdv{2.66} & 4.28\stdv{0.63} \\
        & 3 & 5 & \textbf{99.26}\stdv{0.04} & \textbf{95.00}\stdv{3.61} & \textbf{83.92}\stdv{1.53} & 7.02\stdv{0.53} & \textbf{90.20}\stdv{0.58} & \textbf{7.29}\stdv{0.49} & 73.48\stdv{2.70} & \textbf{10.05}\stdv{2.35} \\

\bottomrule
\end{tabular}}
\vspace{0.2cm}
\caption{Bias-conflicting data detection performance. We report AUROC and AUPRC measured by varying ensemble threshold $\rho$ and number of models for ensemble $M$. These results are evaluated on the same bias severity setting (1.0\%). Best performing results are marked in bold.}
\vspace{-1.5cm}
\label{tab:ablation_detection}
\end{table}

==> tables/ablation_ensemble.tex <==
\begin{table}
\begin{center}
\label{table:headings}
\scalebox{1}{
\begin{tabular}{c|ccc}
\toprule 
M &  1  &	5  \\
\midrule
Colored MNIST & XX & xx	  \\

BFFHQ & XX & xx	  \\

Dogs \& Cats  & XX	 & xx \\

BAR & XX & xx	  \\


\bottomrule
\end{tabular}}
\caption{Ablation - ensemble}
\end{center}
\end{table}

==> tables/ablation_threshold_prev.tex <==
\begin{table}
\begin{center}
\label{table:headings}
\resizebox{0.5\linewidth}{!}{
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{c|cccccc}
% \hline\noalign{\smallskip}
\toprule 
Threshold & 0.9	& 0.95  &	0.98 &	0.99 &	0.995 &	0.999 \\
\midrule
Colored MNIST & 0.9	& 0.95  &	0.98 &	0.99 &	0.995 &	0.999 \\

BFFHQ & 0.9	& 0.95  &	0.98 &	0.99 &	0.995 &	0.999 \\

Dogs \& Cats  & 0.9	& 0.95  &	0.98 &	0.99 &	0.995 &	0.999 \\

BAR & 0.9	& 0.95  &	0.98 &	0.99 &	0.995 &	0.999 \\


\bottomrule
\end{tabular}}
\caption{Ablation - threshold}
\label{tab:ablation_threshold}
\end{center}
\end{table}

==> tables/acc_align_conflict.tex <==
\begin{table}[t!]
\begin{center}
\label{table:headings}
\resizebox{0.9\linewidth}{!}{
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{c|ccc|cc|cc}
% \hline\noalign{\smallskip}
\toprule 
Metric & \multicolumn{3}{c}{Accuracy} & \multicolumn{2}{c}{\# of B.A.(\%)$\uparrow$} & \multicolumn{2}{c}{\# of B.C.(\%)$\downarrow$}\\
% \midrule
\cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Method & LfF & \multicolumn{2}{c}{LfF+BE} & \multicolumn{2}{c}{LfF+BE} & \multicolumn{2}{c}{LfF+BE} \\
% \midrule
\cmidrule(lr){1-1}\cmidrule(lr){2-2} \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
$M$ & - & 1 & 5 & 1 & 5 & 1 & 5 \\
\midrule
Colored MNIST & 76.81\stdv{4.56} & 79.51\stdv{1.56} & \textbf{81.17}\stdv{0.68} & 84.10\stdv{11.01} & 99.96\stdv{0.03} & 4.64\stdv{0.79} & 1.42\stdv{0.78} \\

BFFHQ         & 69.24\stdv{2.07} & 71.52\stdv{2.68} & \textbf{75.08}\stdv{2.29} & 84.51\stdv{4.34} & 92.22\stdv{0.26} & 24.47\stdv{4.63} & 24.37\stdv{3.07} \\

Dogs \& Cats  & 71.72\stdv{4.56} & 76.98\stdv{6.63} & \textbf{81.52}\stdv{1.13} & 85.89\stdv{2.61} & 88.60\stdv{1.02} & 12.00\stdv{6.25} & 9.50\stdv{3.75} \\
    
BAR           & 70.16\stdv{0.77} & 71.63\stdv{1.59} & \textbf{73.36}\stdv{0.97} & 97.24\stdv{0.27} & 98.39\stdv{0.19} & 60.00\stdv{13.24} & 51.42\stdv{5.34} \\

\bottomrule
\end{tabular}}
\vspace{0.5cm}
\caption{
    Unbiased test set accuracies on 1) LfF, 2) applying BE on LfF with a single BCD and 3) multiple BCDs. 
    $M$ indicates the number of BCDs when using BE.
    Best performing results are marked in bold.
    The remaining number of bias-aligned samples~(abbreviated as \# of B.A.) and bias-conflicting ones~(abbreviated as \# of B.C.) in the bias-amplified dataset $\mathcal{D}_A$ after applying BE.
    The remaining numbers are shown in ratios of samples compared to the original training dataset $\mathcal{D}$.
    }
\label{tab:ablation_threshold}
\vspace{-1.0cm}
\end{center}
\end{table}

% Threshold & 0.9	& 0.95  &	0.98 &	0.99 &	0.995 &	0.999 \\
% \midrule
% Colored MNIST & 0.9	& 0.95  &	0.98 &	0.99 &	0.995 &	0.999 \\

% BFFHQ & 0.9	& 0.95  &	0.98 &	0.99 &	0.995 &	0.999 \\

% Dogs \& Cats  & 0.9	& 0.95  &	0.98 &	0.99 &	0.995 &	0.999 \\

% BAR & 0.9	& 0.95  &	0.98 &	0.99 &	0.995 &	0.999 \\

==> tables/main_best_test_acc.tex <==
\begin{table*}
\begin{center}
% \vspace{-0.3cm}
\resizebox{0.8\linewidth}{!}{
\setlength{\tabcolsep}{0.5em}
\def\arraystretch{1.6}% 
\begin{tabular}{cccccccccc|cccc}
% \hline\noalign{\smallskip}
\toprule 
\multirow{2.5}{*}{\large Dataset} 
& \multirow{2.5}{*}{\large Ratio (\%)} 
% & \multirow{2.5}{*}{\large Ratio} 
&
& Vanilla~\cite{He2015resnet}
& HEX~\cite{wang2018hex}
& LNL~\cite{LNL}
& EnD~\cite{EnD}
& ReBias~\cite{bahng2019rebias}
& LfF~\cite{nam2020learning}
& DisEnt~\cite{disentangled}
& \multicolumn{2}{c}{LfF+BE}
& \multicolumn{2}{c}{DisEnt+BE}
\\
\cmidrule{4-14}
&&
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldxmark}
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldcheckmark}
& \textcolor{black}{\boldcheckmark} \textcolor{black}{\boldcheckmark}
& \textcolor{black}{\boldcheckmark} \textcolor{black}{\boldcheckmark}
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldcheckmark}
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldxmark}
& \textcolor{black}{\boldxmark} \textcolor{black}{\boldxmark}
& \multicolumn{2}{c}{\textcolor{black}{\boldxmark} \textcolor{black}{\boldxmark}}
& \multicolumn{2}{c}{\textcolor{black}{\boldxmark} \textcolor{black}{\boldxmark}}
\\
\midrule
% \multirow{4}{*}{\makecell{\large Colored MNIST}} 
\multirow{4}{*}{\large Colored MNIST}
& {\large 0.5} & & {\large 34.75} & {\large 42.25} & {\large 36.29} & {\large 35.33} & {\large 60.86} & {\large 63.55} & {\large 68.49} & {\large 69.70} & \cellcolor{Gray}(+ 6.15) & {\large \textbf{71.34}} & \cellcolor{Gray}(+ 2.85)  
\\
& {\large 1.0} & & {\large 51.14} & {\large 47.02} & {\large 49.48} & {\large 48.97} & {\large \textbf{82.78}} & {\large 76.81} & {\large 79.99} & {\large 81.17} & \cellcolor{Gray}(+ 4.36) & {\large 82.11} & \cellcolor{Gray}(+ 2.12)
\\
& {\large 2.0} & & {\large 65.72} & {\large 72.82} & {\large 63.30} & {\large 67.01} & {\large \textbf{92.00}} & {\large 84.18} & {\large 84.09} & {\large 85.20} & \cellcolor{Gray}(+ 1.02) & {\large 84.66} & \cellcolor{Gray}(+ 0.57)
\\
& {\large 5.0} & & {\large 82.82} & {\large 85.50} & {\large 81.30} & {\large 82.09} & {\large \textbf{96.45}} & {\large 89.65} & {\large 89.91} & {\large 90.04} & \cellcolor{Gray}(+ 0.39) & {\large 90.15} & \cellcolor{Gray}(+ 0.24) 
\\
\midrule
% \multirow{4}{*}{\makecell{\large BFFHQ}} 
\multirow{4}{*}{\large BFFHQ}
& {\large 0.5} & & {\large 55.64} & {\large 56.96} & {\large 56.88} & {\large 55.96} & {\large 55.76} & {\large 65.19} & {\large 62.08} & {\large 67.36} & \cellcolor{Gray}(+ 2.17) & {\large \textbf{67.56}} & \cellcolor{Gray}(+ 5.48)
\\
& {\large 1.0} & & {\large 60.96} & {\large 62.32} & {\large 62.64} & {\large 60.88} & {\large 60.68} & {\large 69.24} & {\large 66.00} & {\large \textbf{75.08}} & \cellcolor{Gray}(+ 5.84) & {\large 73.48} & \cellcolor{Gray}(+ 7.48)
\\
& {\large 2.0} & & {\large 69.00} & {\large 70.72} & {\large 69.80} & {\large 69.72} & {\large 69.60} & {\large 73.08} & {\large 69.92} & {\large \textbf{80.32}} & \cellcolor{Gray}(+ 7.24) & {\large 79.48} & \cellcolor{Gray}(+ 9.56)
\\
& {\large 5.0} & & {\large 82.88} & {\large 83.40} & {\large 83.08} & {\large 82.88} & {\large 82.64} & {\large 79.80} & {\large 80.68} & {\large \textbf{85.48}} & \cellcolor{Gray}(+ 5.68) & {\large 84.84} & \cellcolor{Gray}(+ 4.16)
\\
\midrule
% \multirow{2}{*}{\makecell{\large Dogs \& Cats}} 
\multirow{2}{*}{\large Dogs \& Cats}
& {\large 1.0} & & {\large 48.06} & {\large 46.76} & {\large 50.90} & {\large 48.56} & {\large 48.70} & {\large 71.72} & {\large 65.74} & {\large \textbf{81.52}} & \cellcolor{Gray}(+ 9.80) & {\large 80.74} & \cellcolor{Gray}(+ 15.00) 
\\
& {\large 5.0} & & {\large 69.88} & {\large 72.60} & {\large 73.96} & {\large 68.24} & {\large 65.74} & {\large 84.32} & {\large 81.58} & {\large \textbf{88.60}} & \cellcolor{Gray}(+ 4.28) & {\large 86.84} & \cellcolor{Gray}(+ 5.26) 
\\
\midrule
% \multirow{2}{*}{\makecell{\large BAR}} 
\multirow{2}{*}{\large BAR}
& {\large 1.0} & & {\large 70.55} & {\large 70.48} & {\large 70.65} & {\large 71.07} & {\large 73.04} & {\large 70.16} & {\large 70.33} & {\large \textbf{73.36}} & \cellcolor{Gray}(+ 3.20) & {\large 73.29} & \cellcolor{Gray}(+ 2.96) 
\\
& {\large 5.0} & & {\large 82.53} & {\large 81.20} & {\large 82.43} & {\large 82.78} & {\large 83.90} & {\large 82.95} & {\large 83.13} & {\large 83.87} & \cellcolor{Gray}(+ 0.92) & {\large \textbf{84.96}} & \cellcolor{Gray}(+ 1.83) \\


\bottomrule
% \vspace{-0.2cm}
\end{tabular}
}
% \vspace{-0.8cm}
\caption{Image classification accuracies on unbiased test sets with varying ratios of bias-conflicting samples. We intentionally omit the standard deviation due to the page limit which we include in the Supplementary.
The \textit{cross} and \textit{check} represent whether each model 1) uses bias labels during training and 2) requires predefined bias type.
For applying BE on LfF and DisEnt, the performance gains are shaded in grey.
Best performing results are marked in bold.}
\label{tab:best_test}
\end{center}
\end{table*}

==> tables/supp_JTT.tex <==
\begin{table}[t]
\centering
% \vspace{-0.1cm}
\resizebox{1.0\linewidth}{!}{
% \setlength{\tabcolsep}{1.0em}
\begin{tabular}{c | c c c c}
% \hline\noalign{\smallskip}
\toprule 
Method & Colored MNIST & BFFHQ & Dogs \& Cats & BAR \\
\midrule
JTT~\cite{jtt} & 74.36\stdv{5.06} & 60.78\stdv{2.62} & 66.38\stdv{8.22} & 71.70\stdv{0.53} \\
\midrule
\multirow{2}{*}{JTT + Ours} & \textbf{78.88}\stdv{2.64} & \textbf{64.96}\stdv{1.50} & \textbf{82.91}\stdv{1.97} & \textbf{73.32}\stdv{0.53} \\ 
 & \cellcolor{Gray} (+4.52) & \cellcolor{Gray} (+4.18) & \cellcolor{Gray} (+16.53) & \cellcolor{Gray}(+1.62) \\

\bottomrule
\end{tabular}}
\vspace{-0.2cm}
\caption{ Comparisons of unbiased test set accuracies of JTT trained with and without our approach. We use 1\% ratio of bias-conflicting samples for each dataset. The performance improvements are shaded in grey.
}
\label{tab:supp_JTT}
\end{table}

